On the quantum cohomology of adjoint varieties

We study the quantum cohomology of quasi-minuscule and quasi-cominuscule homogeneous spaces. The product of any two Schubert cells does not involve powers of the quantum parameter higher than 2. With the help of the quantum to classical principle we give presentations of the quantum cohomology algebras. These algebras are semi-simple for adjoint non coadjoint varieties and some properties of the induced strange duality are shown.

==> combinatoire.tex <==
\section{Rational curves on homogeneous spaces}

\subsection{General definitions}

Let $X$ be a variety with Picard group ${\rm Pic}(X)=\Z$. We shall assume that 
the variety is covered by curves and even rationally connected: any two points 
lie on a connected chain of rational curves. For example any Fano variety 
satisfies this property. We will however apply the following definitions 
to the more restricted case of rational homogeneous spaces.

\begin{defi}
Let $d$ be an integer and $x$ and $y$ be points in $X$. 

(\i) We define $X_d(x)$ to be the locus of points in $X$ connected to $x$ 
by a rational curve of degree $d$:%. In symbols:
$$X_d(x)=\{z\in X\ /\ \textrm{there exists $C$ a rational degree $d$ 
curve through $x$ with $z\in C$}\}.$$

(\i\i) We define $Y_d(x,y)$ to be the locus of points in $X$ connected to $x$ 
and $y$ by the same rational curve of degree $d$. In symbols:
$$Y_d(x,y)=\{z\in X\ /\ \textrm{there exists $C$ a rational degree $d$ 
curve through $x$ and $y$ with $z\in C$}\}.$$

(\i\i\i) We define the invariant $\dmax(X)$ (also denoted $\dmax$) as 
follows:
$$\dmax(X)=\max_{x\in X}(\min\{d\geq0\ /\ X_d(x)=X\}).$$
\end{defi}

We observed in \cite{CMP1} that, for $X$ a minuscule or cominuscule rational 
homogeneous space, the geometry of rational curves and especially the 
geometry of the varieties $X_d(x)$ and $Y_d(x,y)$ is intimately related 
to the quantum cohomology of $X$. We want to develop this relationship to 
any rational homogeneous space with Picard number $\Z$. However, we shall see
that the relationship will be more complicated and even the geometry of the 
varieties $X_d(x)$ and $X_d(x,y)$ becomes more complicated (but also richer) 
in general. 

From now on we assume that $X$ is a rational homogeneous space 
with ${\rm Pic}(X)=\Z$ under a semi-simple group $G$. We fix $T$ a maximal 
torus and $B$ a Borel subgroup of $G$ containing $T$. We denote with 
$\varpi$ the fundamental weight corresponding to $X$, with $P$ the associated 
maximal parabolic subgroup containing $B$ and with $V=V(\varpi)$ the 
irreducible representation of highest weight $\varpi$. For $\eta$ a weight of 
the representation $V$, we denote with $x_\eta$ a vector of weight $\eta$.
All points in $X$ are equivalent 
and we therefore will often take $x_\varpi$, a highest weight vector of $V$,
as general point in $X$ (recall that $X$ is the orbit of $[x_\varpi]$, 
the class of $x_\varpi$ in $\p V$). 

\subsection{First properties of $X_d(x)$ and $Y_d(x,y)$}

%As $X$ is homogeneous, all the varieties $X_d(x)$ are isomorphic. We shall 
%denote the abstract corresponding variety with $X_d$. The point 
%$x_\varpi$ is fixed by the Borel subgroup $B$, therefore, the variety 
%$X_d(x_\varpi)$ is $B$-stable for all $d$. It is a union of Schubert varieties

We introduce the notation $M_{d,3}(X)$ to denote the moduli 
space of degree $d$ morphism from $\pu$ to $X$ with three marked points 
on $\pu$. Recall from \cite{thomsen} or \cite{perrin} that $M_{d,3}(X)$ is 
irreducible smooth and of expected dimension $\dim(X)+dc_1(X)$. In 
particular, we may speak of general degree $d$ rational curves on $X$.
We shall denote by $ev_i:M_{d,3}(X)\to X$ the evaluation map defined by the 
$i$-th marked point.

\begin{prop}      \label{prop_irreductibilite}
Let $x,y$ be two generic points on a generic curve of degree $d$,
then $X_d(x)$ and $Y_d(x,y)$ are irreducible.
\end{prop}

\begin{proo}
We know that $M_{d,3}(X)$ is irreducible. We have a $G$-equivariant 
evaluation $ev_1 : M_{d,3}(X) \to X$. As $X$ is covered by rational 
curves of any degree, its image is $X$ itself. Assume that $x=x_\varpi$.
Let $U$ be a unipotent subgroup such that $U \to X$ is an isomorphism 
from $U$ to an open neighbourhood of $x$, which we denote with $O$.
We have an isomorphism
$$
\begin{array}{rcl}
ev_1^{-1}(x_\varpi) \times U  & \rightarrow & ev_1^{-1}(O) \\
(f,u)  &  \mapsto  &  u \circ f
\end{array}
$$
Since $ev_1^{-1}(O)$, an open subset of $M_{d,3}(X)$, is irreducible,
$ev_1^{-1}(x)$
must be also irreducible. Therefore its image under
$ev_2$ which is $X_d(x_\varpi)$, is irreducible.

For $Y_d(x,y)$ we argue essentially in the same way. We may assume that 
$x=x_\varpi$. We note that $X_d(x_\varpi)$ is a Schubert variety since 
it is irreducible from the above and $B$-stable since $x_\varpi$ is fixed by 
$B$. Because $y$ and the degree $d$ curve through $x_\varpi$ are supposed to 
be general, we may assume that $y$ is in the open $B$-orbit of $X_d(\varpi)$.
Thus there is again a unipotent subgroup $U$ of $B$ such that $U \to X$ 
induces an isomorphism between $U$ and an open neighbourhood of $y$ in 
$X_d(x_\varpi)$. Since $U$ is included in $B$ it preserves 
$ev_1^{-1}(x_\varpi)$, and thus induces an isomorphism
$ev_1^{-1}(x_\varpi) \simeq (ev_1 \times ev_2)^{-1}(x_\varpi,y) \times U$.
Therefore $(ev_1 \times ev_2)^{-1}(x_\varpi,y)$ is irreducible and we 
conclude as before.
\end{proo}

Note that the proof shows that $Y_d(x,y)$ does not depend, up to isomorphism,
on the choice of the two points $x,y$ on a generic curve of degree $d$. Thus
we can define the following:

\begin{defi}
\label{defi_x(2)} Let $X_d$ (resp. $Y_d$) be the isomorphism
class of the varieties $X_d(x)$ (resp. $Y_d(x,y)$) for one (resp.
two) generic point(s) $x$ (resp. $x$ and $y$) on a generic degree $d$ curve.
\end{defi}

We have the following easy

\begin{coro}
The variety $X_d$ in $X$ is a Schubert variety stable under
$P$.
\end{coro}

We shall denote with $x_\varpi(d)$ the $T$-stable point in the open $B$-orbit 
of the Schubert variety $X_d(x_\varpi)$. We define the following invariant:

\begin{defi}
For $d,n$ integers we denote with $\delta_{X}(d,n)$ the dimension of the
space of degree $d$ curves passing through $n$ generic points of a 
generic curve of degree $d$ in $X$.
\end{defi}

For example, the value of $\delta_{\p^k}(1,n)$ is $2(k-1)$ if $n=0$, it is 
$k-1$ if $n=1$, and it is 0 otherwise. We now prove a formula involving 
the dimension of $X_d(x)$ and of $Y_d(x,y)$. 

\begin{prop}      \label{prop_dim_yd}
Let $x,y$ be two generic points on a generic degree $d$ curve, then we 
have 
$$\dim(X_d(x)) + \dim(Y_d(x,y)) + \delta(d,3) = c_1d.$$
\end{prop}

(vrai Fano ICI BOF que veut dire generic degree $d$ curve...la dimension 
de l'espace des modules est par necessairement la dimension attendue...)

\begin{proo}
The moduli space $M_{d,3}(G/P)$ has dimension
$\dim(X) + dc_1$. Therefore, as $X$ is covered by rational curves of any 
degree, the inverse image
$ev_1^{-1}(x_\varpi)$ has dimension
$dc_1$. Considering the morphism
$ev_2 : ev_1^{-1}(x_\varpi) \rightarrow X$, with image $X_d(x_\varpi)$, 
we deduce the following equality of dimensions: 
$\dim((ev_1\times ev_2)^{-1}(x_\varpi,x_\varpi(d)) = c_1 d - \dim(X_d)$.

Now the image of $ev_3 : (ev_1\times ev_2)^{-1}(x_\varpi,x_\varpi(2))
\rightarrow X$ is by definition $Y_d(x,y)$, and the fibers of this 
morphism are $\delta(d,3)$-dimensional.
\end{proo}

\centerline{*************** ICI ENLEVER ? ****************}

\begin{prop}      \label{prop_o2}
Assume that $\delta(d,3)=0$, let $f:\p^1 \rightarrow G/P$ be a smooth curve
containing $x$
and $y$ and assume that $X_d(2)$ is smooth along $f(\p^1)$. Then
$f^* TX_d(2) = {\cal O}(2)^{\oplus \dim X_d(2)}$.
\end{prop}
(vrai Fano)
\begin{proo}
Let $H$ denote the scheme of morphisms $f$ of degree $d$ from $\p^1$ to
$G/P$ such that
$f(0) = x$ and $f(\infty) = y$.
We have $T_{[f]}H \simeq H^0(\p^1,f^*TX(-2))$.
Moreover, since $\delta(d,3) = 0$, the dominant evaluation
morphism $H \to X_d(2)$ is generically
finite, and thus the corresponding tangent map is generically injective.
Therefore for generic $u \in \p^1$ the evaluation map
$H^0(\p^1,f^*TX(-2)) \to T_{f(u)} G/P(-2),s \mapsto s(u)$ is injective.
Note that by definition of $X_d$, $s(u)$ in fact lies in $T_{s(u)} X_d(2)$.

Denoting $Y = X_d(2)$,
we thus have a generically injective morphism of $\co_{\p^1}$-sheaves
$$ H^0(\p^1,f^*TX(-2)) \otimes {\cal O}_{\p^1}  \to  f^* TY(-2).  $$
It must therefore be injective. Let $C = f(\p^1)$. The dimension of the
space of curves included in
$Y$ is $\dim Y + \scal{C,c_1(Y)}$, which is well-defined since $Y$ is
smooth along $C$, and is at most $3 \dim Y$ since $\delta(d,3) = 0$ (the fibers
of $M_{d,3}(Y) \to Y^3$ are thus 0-dimensional).
Thus $\scal{C,c_1(Y)} \leq 2 \dim Y$ and the bundle on the right
has non positive degree. Therefore
the morphism of $\co_{\p^1}$-modules is an isomorphism.
\end{proo}

\begin{coro}      \label{coro_yd_independant}
In the conditions of proposition \ref{prop_o2}, for generic $u,v \in X_d(x,y)$,
we have $X_d(u,v)=X_d(x,y)$.
\end{coro}
\begin{proo}
Let $ev_{1,2,3} : M_{d,3}(X_d(x,y)) \to X_d(x,y)^3$.
By proposition \ref{prop_o2} these varieties
have the same dimension and since $\delta(d,3)=0$ this morphism
is generically finite.
Therefore it is dominant. Thus for generic $u,v,w \in X_d(x,y)^3$
there is a curve of degree
$d$ in $X_d(x,y)$ through $u,v$ and $w$.
This implies that $w \in X_d(u,v)$. Thus
$X_d(x,y) \subset X_d(u,v)$. Since by proposition \ref{prop_irreductibilite},
$X_d(u,v)$ is irreducible,
we have equality.
\end{proo}

\centerline{*************** ICI ENLEVER ? ****************}

\subsection{Explicit description of $X_d$ and $Y_d$}

In this section, we describe combinatorially what we expect the 
varieties $X_d$ and $Y_d$ should be. We shall prove in this article that 
this description is valid for minuscule, cominuscule, adjoint and coadjoint 
varieties. We shall study the general geometry of the varieties $X_d$ and 
$Y_d$ and relate them to quantum cohomology in a forthcomming paper 
\cite{fourre-tout}. 

\subsubsection{A combinatorial algorithm}
\label{algo}

Let $d$ be an integer, we describe an algorithmic procedure to
construct from $d$, the root system $R$ of $G$ and the fundamental 
weight $\varpi$ a sequence $(\theta_i,d_i)_i$ where $(\theta_i)_i$ 
is a family of orthogonal roots and $d_i$ are non negative integers:
\begin{itemize} 
\item $\theta_1$ is the highest
root such that $\scal {\alpha^\dual , \varpi} \leq d$ (we shall see
in Lemma \ref{lemm_theta_d} that this root exists and is unique),
$d_1 = \scal {\alpha^\dual , \varpi}$, and
\item $(\theta_2,d_2),\ldots(\theta_k,d_k)$ is the sequence obtained by
the irreducible root system orthogonal to $\theta_1$ containing the
root dual to $\varpi$, the restriction of $\varpi$ to this root
system and the integer $d - d_1$ (this process stops when the root
system is empty or $d=0$).
\end{itemize} 
We denote with $k$ the number of roots obtained and 
$ \theta(d) := \sum_1^k \theta_i $. We also define the elements $w_d$ of 
the Weyl group by $w_d=s_{\theta_1}\cdots s_{\theta_k}$ (remark that 
these reflections commute). 

\begin{defi}
  For all $d$ large enough, the algorithm produces always the same 
sequence. Let $d$ be large, we denote with $\dmax^{\rm alg}(X)$ the 
integer 
$$\dmax^{\rm alg}(X)=\sum_{i=1}^k d_i.$$ 
%where the $d_i$'s are
%the numbers obtained in the previous sequence for $R$, $\varpi$ and
%large values of $d$.
\end{defi}
%, where $R$ is the root system of $G$ and
%$\omega$ is the minimal weight of an equivariant projective
%embedding of $G/P$. 

%Let us assume that $d = \sum d_i$. 
By proposition \ref{prop_chaine} below, the sequence 
$(\theta_i , d_i)_{i\in[1,k]}$ defines a chain of rational curves of 
degree $d_i$, connecting $x_\omega$ and $x_{w_d(\varpi)}$.
%\omega - \sum d_i \theta_i}$. 
We may now state our first conjectural results on $X_d$, $Y_d$ and the 
geometry of rational curves on $X$:

\begin{conj}
\label{conj} 
~

(\i) We have $\dmax(X)=\dmax^{\rm alg}(X)$.

(\i\i) The variety $X_d$ is isomorphic to $X(w_d)$.
\end{conj}

%Une des difficultes ici est de calculer la dimension de la variete
%$X_d(1)$ (ainsi que celle de $X_d(2)$). Il y a pas mal d'exemples ou
%on sait faire marcher les choses (notamment dans le cas des groupes
%classiques c'est vrai) mais en general on ne sait pas calculer ces
%dimensions proprement (ce qui est grosso modo equivalent a donner
%une decomposition de $f^*T_X$).

\subsubsection{Description of $X_d$ and $Y_d$ for small degrees}

%Recall the definition of $X_d(1)$ and $X_d(2)$ (definition
%\ref{defi_x(2)}). Let $\omega$ be the fundamental weight such that
%$G/P \subset \p V_\omega$ and l
Let $\Theta$ denote the highest root
of $G$. Because $\varpi$ is a fundamental weight, we may define its dual 
fundamental weight $\varpi^\vee$. We have the following description of 
$Y_d$ for small degree $d$:

\begin{prop}
\label{prop_yd_courbe}
Let $d \leq (\varpi^\vee , \Theta)$.
Then $Y_d$ is a rational curve of degree $d$.
\end{prop}

Before we proceed to the proof, let us recall what $T$-invariant chains
of rational curves are described as follows (see for example \cite{FW}):

\begin{prop}      \label{prop_chaine}
The chains of $T$-invariant $k$ rational curves starting from $x_\varpi$ 
with degrees $d_1,\ldots,d_k$ are in bijection
with the sequences $(\alpha_k , \alpha_{k-1} , \ldots , \alpha_1)$
of positive roots with $\scal{s_{\alpha_{m-1}} \cdots 
s_{\alpha_1}(\varpi) , \alpha_m^\vee}
= d_m $.

The end-point of the $m$-th component of such a chain is the projectivisation
of the weight line of weight
$s_{\alpha_m} \cdots s_{\alpha_1}(\varpi) =
\varpi - d_1 \alpha_1 - \cdots - d_m \alpha_m$.
\end{prop}

\begin{prooprop}\
ICI REVOIR...
We consider a sequence of roots $(\alpha_1,\ldots,\alpha_k)$ as described 
in Proposition
\ref{prop_chaine} and we denote with $d_i$ the degree of the
$i$-th component of this chain.
We have the equalities $d_i = \scal { s_{\alpha_{i-1}} \cdots 
s_{\alpha_1}(\varpi) ,\alpha_i^\vee }
= \scal { \varpi- d_1 \alpha_1 - \cdots - d_{i-1} \alpha_{i-1} ,
  \alpha_i^\vee }$
thus $\scal{\alpha_i^\vee , \omega} = d_i + \sum_{j<i} d_j
\scal{\alpha_i^\vee ,
\alpha_j}$.
Therefore we get:
$$
\scal{\varpi^\vee - s_{\alpha_k} \cdots s_{\alpha_1}(\varpi^\vee)
, \varpi} = \sum d_i \scal { \alpha_i^\vee , \varpi } = \sum d_i^2 + 
\sum_{i>j} d_id_j \scal{\alpha_i^\vee , \alpha_j} \leq (\sum d_i)^2 = d^2.$$
That is to say, the endpoint of such a chain is not greater than the 
endpoint of an irreducible curve of degree $d$. Moreover, equality in the 
above sequence of inequalities implies that $\scal { \alpha_i^\vee , 
\alpha_j } = 2$, or $\alpha_i = \alpha_j$, a contradiction. This and 
Proposition \ref{prop_irreductibilite} also proves that there is a maximal 
root $\alpha$ among those with $(\varpi,\alpha) = d$; we denote it with 
$\theta_d$.

So each chain of $T$-stable curves whose total degree is $d$ from 
$x_\varpi$ to $x_d$ must be the irreducible curve given by $\theta_d$, and this
proves that $X_d(x,y)$ is
this rational curve.
\end{prooprop}

\begin{coro}
Conjecture \ref{conj} is true for $d\leq (\omega^\dual,\theta)$.
\end{coro}

\begin{proo}
Obviously the Schubert variety $X(x_{w-\sum d_i\theta_i})$ is
contained in $X_d(x_\omega)$. Its dimension is the $P$-length of
$s_{\theta_d}$ (where $X=G/P$). A case by case check (encore
malheureusement) gives
$$\ell_P(s_{\theta_d})=c_1d-1.$$
The result follows by dimension count.
\end{proo}

%Note that this Proposition prove conjecture \ref{conj} for
%$d\leq\sca{\theta}{\omega^\dual}$.
Note that during the proof of
the proposition, the following fact was established~:

\begin{lemm}        \label{lemm_theta_d}
Let $R$ be a root system, $\omega$ a weight and $d$ an integer. There is a
maximal root along those with $\scal{\omega^\dual , \alpha} \leq d$.
\end{lemm}

As an evidence for Conjecture \ref{conj}, we note prove the following
combinatorial result (which is a direct consequence of the conjecture):

\begin{prop}
  Let $(\theta_1,\cdots,\theta_k)$ be the sequence obtained by the
  algorithm for large degrees. Define the element
  $v=s_{\theta_1}\cdots s_{\theta_k}$ of the Weyl group. Let $P$ be
  the maximal parabolic subgroup associated to $\omega$ and $X^P(v)$
  the Schubert variety in $G/P$ associated to $v$.
Then $X^P(v)=G/P$.
\end{prop}

\begin{proo}
We will not deal with the root systems of type $B$, $D$ and $G_2$
where some technical problems make the proof more longer. These cases
can be checked directly (ICI, comme les autres d'ailleurs...).

We shall need the following observations on the sequence of roots
$(\theta_i)$. First remark that because $d$ is large, all these roots
are highest root for an irreducible root system. Furthermore, the root
systems in which they are an highest root being decreasing, we have
$\theta_i\geq\theta_{i+1}$ (where the inequality means that all the
coefficients in the writing as a sum of simple roots are bigger).

Let us now recall the following general principle on the highest root of a
root system. Let $R$ be an irreducible root system different from
$A_1$ and let $\theta$ be its highest root. A simple root $\a_\theta$
non othogonal to the highest root $\theta$ is an adjoint simple root
(there is a unique such root except in type $A$ where
there are two of them) and we have
$\sca{\theta^\vee}{\a_\theta}=1$. In type $A_1$, the highest root is
the adjoint root and $\sca{\theta^\vee}{\a_\theta}=2$.

Let us now denote by $R_i$ the root system where the root $\theta_i$
is an highest root. Remark that $R_i$ can be of type $A_1$ only
 if $i=k$. By construction, an adjoint root $\a_{\theta_i}$
for this system is not in the root system $R_{i+1}$ thus its
intersection with $\theta_{i+1}$ is negative. Furthermore, we
have $\sca{\theta_{i+1}^\vee}{\a_{\theta_i}}=-1$ except in two cases:
$R_i$ of type $B_3$ resp. $G_2$ and $\a_{\theta_i}=\a_2$ in both
cases. These case are excluded.

To prove the proposition, we compute the root $\beta=s_{\theta_1}\cdots
s_{\theta_k}(\a)$ for a simple root $\a$.
% having a positive coefficient on
%$\a_P$. Let $\gamma$ be a simple root in the support of $\a$.

\begin{fact}
The root $\beta$ is negative.
%  The difference $\a-\beta$ is a non negative linear combination of
% simple roots. More precisely, we have the alternative
% \begin{itemize}
% \item $\beta=\a$
%\item $\beta$ is negative.
% \end{itemize}
\end{fact}

\begin{proo}
Let $i$ be the biggest integer such that $\a$ is a root of the root
system $R_i$. Then by construction, for all $j<i$, we have
$\sca{\theta_j^\vee}{\a}=0$. Of course $\a$ is not in the root
systems $R_j$ for $j>i$ and is not adjacent to the root systems
$R_j$ for $j>i+1$. Hence we have $\sca{\theta_j^\vee}{\a}=0$ for
$j>i+1$. Because the roots $\theta_j$ are all orthogonal we get
$$v(\a)=\a-\sca{\theta_i^\vee}{\a}\theta_i-
\sca{\theta_{i+1}^\vee}{\a}\theta_{i+1}.$$
There may be two cases: if $\sca{\theta_i}{\a}=0$ (this can only
happen in type $B$ or $D$ and when $\a\neq\a_P$ and thus is excluded).
% then $\sca{\theta_{i+1}^\vee}{\a}=0$ and  $v(\a)=\a$.
Otherwise, we have that $\a$ is an
adjoint root in the root system $R_i$. We obtain:
%In all cases except if $R_i$ is
%of type $B_3$ and $G_2$ we have
$$\a-v(\a)=\theta_i-\theta_{i+1}.$$
But $\a$ has positive coefficient in $\theta_i$ and does not appear in
$\theta_{i+1}$. The result follows for these types.
%In type $B_3$ and
%$G_2$ the result follows by an easy check.
In case $i=k$ and $R_k$ is
of type $A_1$, we have $\a=\a_P$ and we get $v(\a)=-\a$.
\end{proo}

To finish the proof,
%let us first say that the $G_2$ case can be
%easily checked by hand.
we only need to prove that for $\a'$ a positive
root containing $\a_P$ the simple root associated to $P$ (or the
simple root dual to $\omega$) we have that $v(\a')$ is a negative root. Let
us compute $v(\a_P)$. By construction $\a_P$ is in all the root
systems $R_i$ and is a adjoint root in the root system $R_k$. In
particular $\sca{\a_P}{\theta_i^\vee}=0$ except for $i=k$ where
$\sca{\theta_k^\vee}{\a_P}=2$ resp. 1 if $R_k$ is of type $A_1$
resp. is not of type $A_1$. We thus have $v(\a_P)=-\a_P$
resp. $v(\a_P)=\a_P-\theta_k$. In the first case $v(\a_P)$ is
negative. In the second case, because $R_k$ is not
of type $A_1$, there is a root different from $\a_P$ is the root
system and $v(\a_P)$ is also negative.

Now write $\a'=\a_P+\a$ where $\a$ is
a non negative linear combination of simple roots. Write $\beta=v(\a)$.
%and $\gamma=\a-\beta$ where $\gamma$ is a
%non negative linear combination of simple roots. Remark that
%$\beta=\a-\gamma$ being a root and because its coefficient with
%respect to $\a_P$ is non positive it is
%being
We get
$$v(\a')=v(\a_P)+v(\a)=v(\a_P)+\beta%\leq av(\a_P)
<0.$$
The result follows.
\end{proo}

















==> general.tex <==
ICI : definir les varietes $Y_d$

\begin{lemm}
\label{lemm-yd-irr}
The variety $Y_d(X)$ is irreducible.
\end{lemm}

==> tableau-e6p2-8-2-1.tex <==
%% GENERATED BY QUIVER CALCULUS


\begin{pspicture*}(0,0)(3.0,2.4)

\psline(0.699,0.099)(1.101,0.501)
\psline(0.501,0.099)(0.099,0.501)
\psellipse(0.6,0.0)(0.14,0.14)
\put(0.54,0.0){4}
\psline(1.101,0.699)(0.699,1.101)
\psline(1.299,0.699)(1.701,1.101)
\psellipse(1.2,0.6)(0.14,0.14)
\put(1.14,0.6){2}
\psline(2.301,0.699)(1.899,1.101)
\psellipse(2.4,0.6)(0.14,0.14)
\put(2.34,0.6){3}
\psline(0.099,0.699)(0.501,1.101)
\psellipse(0.0,0.6)(0.14,0.14)
\put(-0.06,0.6){1}
\psline(0.699,1.299)(1.101,1.701)
\psellipse[fillstyle=solid,fillcolor=black](0.6,1.2)(0.14,0.14)
\psline(1.701,1.299)(1.299,1.701)
\psellipse[fillstyle=solid,fillcolor=black](1.8,1.2)(0.14,0.14)
\psline(1.2,1.94)(1.2,2.26)
\psellipse[fillstyle=solid,fillcolor=black](1.2,1.8)(0.14,0.14)
\psellipse[fillstyle=solid,fillcolor=black](1.2,2.4)(0.14,0.14)

